Value Penalized Q-Learning for Recommender Systems

Scaling reinforcement learning (RL) to recommender systems (RS) is promising since maximizing the expected cumulative rewards for RL agents meets the objective of RS, i.e., improving customers' long-term satisfaction. A key approach to this goal is offline RL, which aims to learn policies from logged data. However, the high-dimensional action space and the non-stationary dynamics in commercial RS intensify distributional shift issues, making it challenging to apply offline RL methods to RS. To alleviate the action distribution shift problem in extracting RL policy from static trajectories, we propose Value Penalized Q-learning (VPQ), an uncertainty-based offline RL algorithm. It penalizes the unstable Q-values in the regression target by uncertainty-aware weights, without the need to estimate the behavior policy, suitable for RS with a large number of items. We derive the penalty weights from the variances across an ensemble of Q-functions. To alleviate distributional shift issues at test time, we further introduce the critic framework to integrate the proposed method with classic RS models. Extensive experiments conducted on two real-world datasets show that the proposed method could serve as a gain plugin for existing RS models.

==> 2.Permilinaries.tex <==
\section{Preliminaries}



\subsection{Interactive Recommendation Problem}
% 目标是依据历史记录推荐下一个最相关的商品


\subsection{MDP on Recommendation Problem}
% 

\subsection{Distributional Shift Issues}


We represent the recommendation problem as a Markov decision process (MDP) defined by a tuple $(\mathcal{S},\mathcal{A}, T, d_0, r, \gamma)$:
\begin{itemize}
\item \textbf{State space} $\mathcal{S}$ is a continuous space describing the user’s interaction history. The interaction sequence contains 10 items the user lastly interacted with. We then use the recommendation model to map it into a latent space as the state for Q heads and as the features for CE head.
\item \textbf{Action space} $\mathcal{A}$ is a finite set of actions of recommendation agents. 
For a state $s_t$, the candidate actions are all items in the dataset. 
\item \textbf{Initial state distribution} $d_0$ is the distribution that initial state follows.
\item \textbf{Transition probability} $T$ is a conditional probability with $T(s_{t+1} | s_t, a_t)$ describing the distribution over the next state $s_{t+1}$ after taking action ${a_t}$ at state $s_t$.
\item \textbf{Reward function} $r$ describes the immediate rewards. For example, agent will get a reward $r(s_t, a_t)$ when taking the action ${a_t}$ at state ${s_t}$. 
\item \textbf{Discount factor} $\gamma$ is a scalar that makes trade-off between immediate rewards and long-term rewards.
\end{itemize}

The goal of reinforcement learning is to find a policy $\pi(a_t|s_t)$, which defines a distribution over actions $a_t$ conditioned on states $s_t$, so as to maximize the cumulative reward:
\begin{equation}
    \mathbb{E}_{\tau \sim p_{\pi}(\tau)} \Big[ \sum_{t=0}^{|\tau|} \gamma^t r(s_t, a_t)\Big],
\end{equation}
\noindent where the trajectory distribution $p_{\pi}$ for a transition probability $T$, a policy $\pi$ and an initial state distribution $d_0$ is:
\begin{equation}
    p_{\pi}(\tau) = d_0(s_0) \prod_{t=0}^{|\tau|} \pi(a_t|s_t) T(s_{t+1}| s_t, a_t)
\end{equation}


\subsection{Value-based RL}
\noindent Value-based RL methods, such as DQN \cite{mnih2015human}, usually try to learn a state-action value function $Q_\theta(s,a)$ with parameter $\theta$,  defined as:
\begin{equation}
    Q^{\pi}(s_t, a_t) = \mathbb{E}_{\tau \sim p_{\pi}} \Big[ \sum_{t'=t}^{|\tau|} \gamma^{t' -t} r(s_{t'}, a_{t'}) \Big]
\end{equation}

An improved policy $\pi^\prime (a|s)$ can be easily obtained by $\pi^\prime (a|s) = \arg \max_{a} Q_\theta (s,a)$. And the parameter $\theta$ for the value network is obtained by minimizing the following loss function with a given dataset $D$:

\begin{equation}
    \mathcal{L}_{\theta} = 
    \frac{1}{2}
    \mathop{\mathbb{E}}\limits_{(s_t,a_t,r_t,s_{t+1}) \sim D} 
    \Big[ \big(
    y_t - Q_{\theta}(s_t, a_t) 
    \big)^2 \Big],
    \label{equation_loss}
\end{equation}

\noindent where the item $y_t = r_t + \gamma \max_{a'}Q_{\theta_T}(s_{t+1}, a')$ is the so called target, and $Q_{\theta_T}$ is the target network with frozen parameters from historical value function $Q_{\theta}$. 

\subsection{Challenges: Distributional Shift in Value-based RL}
A key source of instability of value-based RL methods applying on static datasets is the distributional shift during the training and test phase \cite{levine2020offline}. Distributional shift happens when evaluating a trained policy on another different distribution. It can be categorized into two types: state distribution shift and action distribution shift. Here, we explain these issues within the value-based RL methods. 

State distribution shift affects the performance of RL agents only at test time. 
The learned policy will always meet unseen states at test time since the dataset usually does not fully cover the state space. 
The output of the Q-function can be unstable as the loss function in Equation (\ref{equation_loss}) makes no guarantees about the error when encountering OOD state inputs, resulting in performance degradation at test time \cite{lee2020addressing}.
Unfortunately, the narrow distribution of the collected trajectories in RS datasets and the non-stationary environments exacerbate this problem. 

Action distribution shift affects the agent both at test time and training time. 
The Q-function is trained on dataset state-action pairs but is evaluated on all valid actions for policy improvement and real actions generation.
At test time, the unstable predictions on OOD actions may result in unreasonable actions as the side effect of the greedy policy. 
During training, the highest value among noisy predictions in target will be taken as the future reward and then spread to the learned Q-function, leading to a persistent overestimation bias \cite{jaques2019way, kumar2019stabilizing}. 
In the online setting, active learning around these overestimated state-action pairs would correct them. 
By contrast, such correction will never happen in the offline setting since the agents can no longer interact with the environment. 
Moreover, the large action space in RLRS exacerbates this problem. 
For example, the general RL testbed Arcade Learning Environment \cite{bellemare2013arcade} consists of no more than 18 discrete actions, while the candidate recommending items in the Retailrocket dataset, a real-world commercial dataset, is 70,852 (please refer to Table \ref{dataset_static} for the details). 


==> 3.RelatedWork.tex <==
\section{Related work}
There are several difficulties in building RLRS, such as the state representation \cite{lei2020reinforcement, liu2020state, wang2020kerl}, the slated-based recommendation setting \cite{sunehag2015deep, swaminathan2016off, chen2019top, gong2019exact, ie2019reinforcement} and the large-scale recommendation problem \cite{dulac2015deep, zhao2019deep}. However, there has been limited attention paid to the negative impact of offline setting, i.e., training RLRS agents from static datasets. Here we give a literature review on the general offline RL methods. 

% policy constrain methods
\subsubsection{Constrain Policy Close to the Behavior Policy.} Methods based on different distance metrics are proposed to compel the RL policy close to the behavior policy that produces the dataset \cite{levine2020offline}, such as KL divergence \cite{jaques2019way}, Wasserstein distance \cite{wu2019behavior}, MMD \cite{kumar2019stabilizing}, Fisher divergence \cite{kostrikov2021offline} and Euclidean squared distance \cite{Fujimoto2021AMA}. 
In this approach, GCQ \cite{wang2020off} utilizes a
neural generator to recover the distribution of dataset, which is similar to BCQ \cite{fujimoto2019off}. 
These methods may suffer from estimating the dataset trajectories distribution in RS. 

\subsubsection{Estimate Accurate/Conservative Q-values.} Algorithms like Ensemble-DQN \cite{fausser2015neural, osband2016deep}, QR-DQN \cite{dabney2018distributional}, and REM \cite{agarwal2020optimistic} in this approach estimate Q-values by predicting the expectation of a distribution or an ensemble. Another instance is CQL \cite{kumar2020conservative}, which adds two regularization terms to the Q-function update so as to avoid overestimating OOD actions. Despite its good performance in general RL testbeds, CQL may suffer from high dimensional action space (minimization term in CQL) and non-user trajectories in the datasets (maximization term). 
The proposed VPQ can be categorized into this approach. 
Besides, a recently proposed method named UWAC \cite{yuewu2021} adds uncertainty-aware weights to the Q-function queries, combining the two main approaches.
